BoxVIS: Video Instance Segmentation with Box Annotations

It is expensive and labour-extensive to label the pixel-wise object masks in a video. As a result, the amount of pixel-wise annotations in existing video instance segmentation (VIS) datasets is small, limiting the generalization capability of trained VIS models. An alternative but much cheaper solution is to use bounding boxes to label instances in videos. Inspired by the recent success of box-supervised image instance segmentation, we adapt the state-of-the-art pixel-supervised VIS models to a box-supervised VIS (BoxVIS) baseline, and observe slight performance degradation. We consequently propose to improve the BoxVIS performance from two aspects. First, we propose a box-center guided spatial-temporal pairwise affinity (STPA) loss to predict instance masks for better spatial and temporal consistency. Second, we collect a larger scale box-annotated VIS dataset (BVISD) by consolidating the videos from current VIS benchmarks and converting images from the COCO dataset to short pseudo video clips. With the proposed BVISD and the STPA loss, our trained BoxVIS model achieves 43.2\% and 29.0\% mask AP on the YouTube-VIS 2021 and OVIS valid sets, respectively. It exhibits comparable instance mask prediction performance and better generalization ability than state-of-the-art pixel-supervised VIS models by using only 16\% of their annotation time and cost. Codes and data can be found at \url{https://github.com/MinghanLi/BoxVIS}.

==> figs/mask_box_sup.tex <==
\begin{figure*}
\begin{center}
    \includegraphics[width=1\linewidth]{figs/fig/min_boxvis.jpg}
\end{center}
\vspace{-5mm}
\caption{The relationship between the number of box annotations and segmentation performance. The three makers represent the different number of training samples. $\bigstar$ indicate the isolated training on YTVIS21 or OVIS dataset respectively, $\blacktriangleright$ means the joint training on YTVIS21 and OVIS datasets, and $\blacklozenge$ is the joint training on our proposed JVIS dataset. }
\label{fig:mask_box_sup}
\end{figure*}

==> sec/2_related_works.tex <==
\section{Related Works}

\subsection{Box-supervised Image Instance Segmentation}
BoxCaseg \cite{wang2021boxcaseg} leverages a salience model to generate pseudo object masks for training Mask R-CNN along with the multiple instance learning (MIL) loss.  Recently, BoxInst  \cite{tian2020boxinst} achieves impressive performance by proposing two box-supervised loss items, the projection loss and the pairwise affinity loss. 
BoxLevelSet \cite{li2022boxlevelset} utilizes the traditional level set evolution to predict the object boundaries and instance masks.
DiscoBox \cite{lan2021discobox} and BoxTeacher \cite{cheng2022boxteacher} employ an exponential moving average teacher to produce high-quality pseudo instance masks for introduction the pseudo pixel-wise mask supervision, bringing significant performance improvement.

\input{figs/boxvis_baseline}

\subsection{Pixel-supervised Video Instance Segmentation}
\textbf{Per-frame input based VIS methods.} A popular VIS pipeline \cite{yang2019video, cao2020sipmask,Li_2021_CVPR,liu2021sg,yang2021crossover,QueryInst,ke2021pcan,huang2022minvis,IDOL} is to extend the representative pixel-supervised IIS methods \cite{he2017mask,bolya2019yolact,tian2020conditional,carion2020end,cheng2021mask2former} by adapting a frame-to-frame instance tracker. For example, in \cite{yang2019video,QueryInst,huang2022minvis}, the clues such as category score, box/mask IoU and instance embedding similarity are integrated into the tracker. 
However, these trackers may fail to distinguish instances with similar appearance, resulting in error-prone frame association. Inspired by the contrastive learning \cite{chen2020simplectt, pang2021quasi,khosla2020supervisedctt,wang2021densectt}, IDOL \cite{IDOL} learns discriminative instance embeddings for multiple object tracking frame by frame.
Besides, clip-to-clip trackers \cite{bertasius2020classifying, lin2021video, qi2021occluded} have been proposed via propagating the predicted instance masks from a key frame to other frames.
% including instance masks propagation from each frame to its neighbouring frames or from several selected key frames to all the other frames. 
The commonly used techniques include deformable convolution \cite{bertasius2020classifying,dai2017deformable}, non-local block \cite{lin2021video}, correlation \cite{Li_2021_CVPR,qi2021occluded}, graph neural network \cite{wang2021end}, \etc. 
% By exploiting the temporal redundancy among overlapped frames, clip-to-clip trackers improve much the performance over per-frame methods.

\textbf{Per-clip input based VIS methods.} StemSeg \cite{Athar_Mahadevan20stemseg} first propose a clip-in clip-out VIS pipeline by modeling a video clip as a single 3D spatio-temporal pixel embedding. In recent years, transformer based per-clip methods \cite{wang2020vistr,wu2022trackletquery,hwang2021video,yang2022TempEffi,seqformer} have achieved impressive progress. VisTR \cite{wang2020vistr} views the VIS task as a direct end-to-end parallel sequence prediction problem, but it needs a large memory to store spatio-temporal features. To solve the issue, DETR-based IFC\cite{hwang2021video} transfers inter-frame information via efficient memory tokens, and SeqFormer \cite{seqformer} locates an instance in each frame and aggregates temporal information to predict video-level instances. 
Besides, to keep the temporal consistency, EfficientVIS \cite{wu2022trackletquery} transfers inter-clip query embeddings via a temporal dynamic convolution.

Although the pixel-supervised VIS methods have achieved impressive performance on current VIS benchmarks YTVIS21 and OVIS respectively, but their generalization capability may be limited, because the amount of pixel-wise annotations is small. For example, the VIS model trained only on YTVIS21 dataset fails to handle the videos with crowded objects like OVIS. It is expensive and labour-extensive to label the pixel-wise object masks in a video. Inspired by the successful of box-supervised IIS methods, in this paper we extend the state-of-the-art pixel-supervised VIS methods to their box-supervised counterparts, and propose a box-center guided spatial-temporal pairwise affinity loss to predict instance masks for better spatial and temporal consistency, finally introduce a larger scale box annotated VIS dataset (BVISD) to improve the generalization capability of box-supervised VIS models.

==> sec/backup.tex <==
%---------------------- CoCo -----------------------------
\begin{table*}
\begin{center}
\begin{tabular}{p{0.05\textwidth}<{\centering}p{0.08\textwidth}<{\centering}p{0.09\textwidth}|p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.035\textwidth}<{\centering}|p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.035\textwidth}<{\centering}}
\hline
Sup. & Matcher & Criterion & \multicolumn{6}{c|}{Box} & \multicolumn{6}{c}{Mask}  \\
     & Mask    &  Mask  & AP & AP$_{50}$ & AP$_{75}$ & AP$_s$  & AP$_m$ & AP$_l$ & AP & AP$_{50}$ & AP$_{75}$ & AP$_s$  & AP$_m$ & AP$_l$\\
\hline\hline
\multicolumn{3}{l}{CondInst}\\
Mask       & biou   & bce + dice  & - & - & - & - & - & - & 35.6 & 56.3 & 37.8 & 16.9 & 38.9 & 51.0 \\
Box        & biou   & proj        & - & - & - & - & - & - & 21.2 & 45.2 & 17.7 & 10.0 & 21.4 & 32.5 \\
Box        & biou   & proj + pair & - & - & - & - & - & - & 30.7 & 52.2 & 31.1 & 13.8 & 33.1 & 45.7 \\
% BoxTeacher   
Box        & biou   & ++pseudo    & - & - & - & - & - & - & 34.2 & 56.0 & 35.4 & - & - & - \\
\hline\hline
\multicolumn{3}{l}{Mask2former} \\
Mask       & bce+dice   & bce + dice  & 45.9 & 65.2 & 49.1 & 27.2 & 48.5 & 62.8 & 43.1 & 65.4 & 46.4 & 22.5 & 46.2 & 64.2\\
Box        & proj   & proj        & 43.3 & 61.1 & 46.3 & 24.8 & 46.9 & 59.9 & 33.6 & 56.7 & 34.2 & 15.2 & 36.0 & 52.0 \\
% & box        & proj   & proj + tv  & 44.8 & 64.3 & 47.9 & 26.3 & 48.5 & 61.0 & 35.0 & 59.1 & 35.4 & 16.4 & 37.4 & 53.2 \\
% & box        & proj   & ++EMA      & 45.9 & 64.4 & 49.4 & 26.7 & 49.5 & 63.6 & 37.5 & 60.9 & 38.4 & 18.7 & 39.4 & 57.1 \\
% \cline{2-16} 
Box        & proj    & proj + pair & 45.8 & 64.4 & 49.1 & 27.4 & 49.4 & 61.7 & 37.6 & 60.7 & 39.4 & 19.2 & 40.5 & 55.1 \\
Box        & proj    & +pseudo    & 46.5 & 65.2 & 50.0 & 28.3 & 49.9 & 62.1 & 39.2 & 62.1 & 41.4 & 20.3 & 41.5 & 57.9 \\
\hline
\end{tabular}
\end{center}
\caption{Results on COCO val2017 set. In mask2former, cross-attn module achieves implicitly a pairwise loss in feature similarity, which performs better than the original lab color similarity of BoxInst\cite{tian2020boxinst}. }
\end{table*}


% ------------------------------------------------------------------------
\begin{table*}
\begin{center}
\begin{tabular}{p{0.09\textwidth}<{\centering}p{0.07\textwidth}<{\centering}|p{0.05\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.04\textwidth}<{\centering}|p{0.06\textwidth}<{\centering}p{0.05\textwidth}<{\centering}p{0.05\textwidth}<{\centering}|p{0.06\textwidth}<{\centering}p{0.05\textwidth}<{\centering}|p{0.06\textwidth}<{\centering}}
\hline
\multirow{2}{*}{Methods} & \multirow{2}{*}{Sup.} & \multicolumn{3}{c|}{Training Data} & \multicolumn{3}{c|}{YTVIS21} & \multicolumn{2}{c|}{{ \color{red} OVIS}} & JVIS\\
                         & & ytvis21 & ovis & coco & val-sub & val & val22 & val-sub & val  & val-sub\\
\hline
\multicolumn{2}{l}{MinVIS} \\
\hline
& Mask & $\checkmark$ &   &  & 48.3  & 43.3 & 31.0 & -    & -    & 34.0 \\
& Mask & & $\checkmark$   &  & -     & -    & -    & 21.5 & 28.8 & 13.6 \\
& Mask & 2  & 1 &            & 49.4  & 45.7 & 33.5 & 21.4 & 29.2 & 35.3 \\
& Mask & 2  & 1 & 1          & 51.6  & 46.0 & 29.4 & 23.2 & 30.0 & 36.8 \\
\hline
& Box  & $\checkmark$ &   &   & 46.8 & 40.5 & 25.1 & -    & -    & 31.1 \\
& Box  & & $\checkmark$   &   & -    & -    & -    & 16.7 & 22.0 & 12.8 \\
& Box  & 2  & 1 &             & 48.3 & 42.0 & 26.0 & 18.7 & 23.9 & 33.9 \\
& Box  & 2  & 1 & 1           & 48.9 & 42.8 & 30.4 & 19.2 & 25.0 & 34.4 \\
\hline
\multicolumn{2}{l}{Mask2Former-video} \\
\hline
& Mask & $\checkmark$ &   &   & 47.2  & 43.1 & 33.5  & -    & -    & 31.9 \\
& Mask & & $\checkmark$   &   & -     & -    & -     & 22.7 & 27.9 & 13.7 \\
& Mask & 2 & 1 &              & 50.1  & 43.8 & 31.7  & 22.9 & 30.9 & 35.3 \\
& Mask & 2 & 1 & 1            & 50.3  & 44.7 & 37.5  & 26.1 & 31.8 & 36.6 \\
\hline
& Box  & $\checkmark$ &   &   & 47.8  & 43.1 & 32.8  & -    & -    & 32.5 \\
& Box  & & $\checkmark$   &   & -     & -    & -     & 20.9 & 25.7 & 13.8 \\
& Box  & 2 & 1 &              & 47.5  & 40.3 & 29.7  & 21.8 & 27.9 & 34.2 \\
& Box  & 2 & 1 & 1            & 48.7  & 42.9 & 31.7  & 23.3 & 28.9 & 35.0 \\
\hline
BoxVIS \\
\hline
\multirow{4}{*}{+temp-pair} 
& Box  & $\checkmark$ &   &   & 48.0  &   &   & -    & - \\
& Box  & & $\checkmark$   &   & -     & - & - & 20.7 &   \\
\cline{2-11}
& Box  & 2 & 1 &   & 48.4  &      &      & 21.7 &   \\
& Box  & 2 & 1 & 1 & 48.8  &      &      & 24.2 & 27.9 \\
coco-pse2
& Box  & 2 & 1 & 1 & 48.7  &      &      & 24.7 & 29.0 \\
\hline 
\multirow{2}{*}{+attnst3}
& Box  & 2 & 1 &   & 47.2 &       &      & 23.2 & \\
& Box  & 2 & 1 & 1 & 49.2 & 43.2  & 27.7 & 24.0 & 28.3 \\
\hline  
\end{tabular}
\end{center}
\caption{Results on YouTubeVIS-2021 and OVIS valid sets. YouTubeVIS-2021 with 360p, while OVIS with 480p. The default pseudo coco clip is first resize coco image [400, 500, 600] and crop size (480, 600), while PseClip2 means that resize coco image [600, 700, 800] and crop size (320, 480). The later can produce the pseudo clip with large camera motion.}
\end{table*}


\begin{table*}
\begin{center}
\begin{tabular}{p{0.075\textwidth}<{\centering}p{0.075\textwidth}<{\centering}p{0.095\textwidth}<{\centering}|p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.04\textwidth}<{\centering}|p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.04\textwidth}<{\centering}|p{0.04\textwidth}<{\centering}}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Finetune-VIS} & \multicolumn{5}{c|}{YT21} & \multicolumn{5}{c|}{YT22}  \\
       & Sup. & Data  & AP & AP$_{50}$ & AP$_{75}$ & AR$_1$  & AR$_{10}$ & AP & AP$_{50}$ & AP$_{75}$ & AR$_1$  & AR$_{10}$ & Mean\\
\hline\hline
\multirow{3}{*}{MinVIS} 
& Mask & yt21      & 43.3 & 64.0 & 46.4 & 39.2 & 51.3 & 31.0 & 56.1 & 31.6 & 27.4 & 33.8 & 37.1\\
& Mask & 2yt+1ovis & 45.7 & 65.8 & 50.2 & 39.4 & 51.6 & 33.5 & 55.8 & 32.4 & 28.7 & 38.0 \\
& Mask & ++1coco   & 46.0 & 66.0 & 51.4 & 40.7 & 53.0 & 29.4 & 49.3 & 31.1 & 28.1 & 33.8 \\
\hline
\multirow{3}{*}{MinVIS-box}
& Box  & yt21      & 40.5 & 64.1 & 44.2 & 37.1 & 47.2 & 25.1 & 47.7 & 25.4 & 24.1 & 30.0 & 33.0 \\
& Box  & 2yt+1ovis & 42.0 & 64.1 & 44.0 & 37.7 & 49.3 & 26.0 & 51.1 & 26.7 & 23.1 & 30.1 & 34.0 \\
& box  & ++1coco   & 42.8 & 64.2 & 46.9 & 37.3 & 48.6 & 30.4 & 53.2 & 31.5 & 26.5 & 36.0 \\
\hline\hline
\multirow{3}{*}{M2F-VIS}
& Mask & yt21      & 43.1 & 63.3 & 46.2 & 39.1 & 51.0 & 33.5 & 55.8 & 39.1 & 30.4 & 39.5 \\
& Mask & 2yt+1ovis & 43.8 & 65.5 & 46.7 & 39.6 & 52.0 & 31.7 & 57.2 & 31.4 & 27.1 & 37.7 \\
& Mask & ++1coco   & 44.7 & 64.8 & 48.5 & 39.3 & 52.2 & 37.5 & 61.1 & 38.2 & 32.5 & 44.8 \\
\hline
\multirow{3}{*}{M2F-VIS-box}
& Box  & yt21      & 43.1 & \\
& Box  & 2yt+1ovis & 40.3 & 61.1 & 43.4 & 37.1 & 48.1 & 29.7 & 51.5 & 29.4 & 28.0 & 35.3 & 35.0\\
& Box  & ++1coco   & 42.9 \\

\hline\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Finetune-VIS} & \multicolumn{8}{c}{OVIS}   \\
       & Sup. & Data  & AP & AP$_{50}$ & AP$_{75}$ & AP$_{so}$ & AP$_{mo}$ & AP$_{ho}$ & AR$_1$  & AR$_{10}$ \\
\hline
MinVIS 
& Mask & ovis      & 28.8 & 51.2 & 28.9 & 44.8 & 33.0 & 11.8 & 14.3 & 33.4 \\
\multirow{2}{*}{BoxVIS}
& Box  & ovis      & 22.0 & 41.0 & 20.9 & 39.0 & 27.2 &  6.6 & 12.8 & 26.5 \\
& Box  & 2ovis+1yt & 23.4 & 43.1 & 22.6 & 43.8 & 27.1 &  7.6 & 13.2 & 26.7 \\
\hline
\multirow{2}{*}{BoxVIS-clip}
& Mask & 2yt+1ovis & \\
& Box  & 2yt+1ovis & 27.9 & 49.4 & 28.8 & 45.5 & 32.0 & 10.3 & 14.5 & 32.4 \\
\hline
\end{tabular}
\end{center}
\caption{Results of BoxInst and MinVIS on YouTube-VIS 2021 and 2022 valid sets. }
\end{table*}

\subsection{Coarse-to-fine pairwise affinity loss}
For one of query features denoted as $q$, we reformulate the masked attention \cref{eq:mask-attn} as $X^l_q = \Delta X^l_q + X^{l-1}_q $ , where the derived value is
\begin{align}\label{eq:deltax}
    \Delta X^l_q  := W^l_q V^l = \text{softmax}(\mathcal{M}^{l-1}_{a, q}+q^l{K^l}^T)V^l.
\end{align}
At a specific feature location $(x,y)$, if the predicted mask ${M}^{l-1}_q(x, y) <= 0.5$, then the attention mask $\mathcal{M}^{l-1}_{a,q}(x, y)=-\infty$, finally leading to $W_{q}^l = 0$. This demonstrates that only the features in the activated mask area contributes to the query feature $q$ in the $l$ layer. 
% \begin{equation}
    % W_{n,i}^l = \frac{\exp(\mathcal{M}_{n,i}^l + Q_n^l {K_i^l}^T)}{\sum_{j=1}^{H^lW^l} \exp(\mathcal{M}_{n,j}^l + Q_n^l {K_j^l}^T)} = 0.
% \end{equation}
Therefore, we group the predicted object locations as an activate set 
$\Omega^{l-1}_q := \{(x, y) | M^{l-1}_q(x, y) > 0.5\}.$
Then Eq. (\ref{eq:deltax}) can be reformulated as
\begin{align}
    \Delta X^l_n & = \sum\nolimits_{i \in \Omega^{l-1}_n} W_{n,i}^l V_i^l \nonumber \\
                 & = \sum\nolimits_{i \in \Omega^{l-1}_n} \frac{1} {\sigma_n^l} \exp(Q_n^l {K^l_i}^T) V_i^l
\end{align}
where $\sigma_n^l = \sum_{i \in \Omega^{l-1}_n} \exp(Q_n^l {K_i^l}^T)$, and the normalization scale ensures that the sum of the weights $W_{n,i}^l$ is 1. Actually the derived value is set to a weighted average of the masked features that are predicted as instances in the last decoder layer.

\textbf{3D Total Variation generalization loss.}
We assume that two neighbouring pixels at feature locations $(x_i, y_i), (x_j, y_j)$ have high feature similarity. The 3D total variation norm (3DTV) with an anisotropic version is 
\begin{align}
    L_\text{3DTV} & = | M(x_i+1, y_i,   t_i  )-M(x_i, y_i, t_i)| \nonumber \\
                  & + | M(x_i,   y_i+1, t_i  )-M(x_i, y_i, t_i)| \nonumber \\
                  & + | M(x_i,   y_i,   t_i+1)-M(x_i, y_i, t_i)|
\end{align}

The total training losses can be written as:
\begin{align}
    {L} & = \lambda_1 {L}_{cls} + \lambda_2 {L}_{box\text{-}mask} \nonumber \\
        & =  \lambda_1 {L}_{cls} + \lambda_2 ({L}_{proj} + \gamma L_\text{3DTV} + (1-\gamma) {L}_\text{affinity}).
\end{align}
where $\gamma = 1$ in the first 12 epochs, otherwise $0$.

Since the total training loss has fast convergence, the first 12 epochs employ total variation generalization to split the input image into coarse regions (contributes to \textbf{fast convergence}), while the last 24 epochs employ pairwise affinity loss to encode fine relationships for paired pixels, at least one of which is in the bounding boxes. 


\subsection{Gaussian blur}
The Gaussian blur is a type of image-blurring filter that uses a Gaussian function for calculating the transformation to apply to each pixel in the image. The formula of a Gaussian blur in three dimensions is 
\begin{equation}
    G(d_x, d_y, d_t) = \frac{1}{2\pi \sigma^2} \exp(-\frac{d_x^2+d_y^2+d_t^2}{2\sigma^2}),
\end{equation}
where $d_x, d_y, d_t$ are the distances from the origin to the destination in the horizontal axis, the vertical axis and the temporal axis respectively, and $\sigma$ is the standard deviation of the Gaussian distribution. Values from this distribution are used to build a convolution matrix which is applied to the original image. Each pixel's new value is set to a weighted average of the pixel's neighborhood. The original pixel's value receives the heaviest weight (having the highest Gaussian value) and neighboring pixels receive smaller weights as their distance to the original pixel increases.

\subsection{Masked-attention}
The masked attention modulates the attention matrix via
\begin{align}
    X^l = \text{softmax}(\mathcal{M}_a^{l-1}+Q^l{K^l}^T)V^l+X^{l-1},
    \label{eq:mask-attn}
\end{align}
where the attention mask $\mathcal{M}_a^{l-1}$ at feature location $(x,y)$ is 
\begin{equation}
    \mathcal{M}_a^{l-1}(x,y) = 
        \begin{cases}
            0,        & \text{if}\ M^{l-1}(x,y) > 0.5, \\
            -\infty,  & \text{otherwise}.  
        \end{cases}   
\end{equation}  
Here, $l$ is the layer index, $X^l \in R^{N\times C}$ refers to $N$ $C$-dimensional query features at the $l^{th}$ layer and $Q^l=f_Q(X^{l-1}) \in R^{N\times C}$. $K^l, V^l \in R^{H^l W^l\times C}$ are the image features under transformation $f_K(\cdot)$ and $f_V(\cdot)$ respectively, and $H^l$ and $W^l$ are the spatial resolution of image features. $f_Q, f_K, f_V$ are linear transformations.


\subsection{Mask generation}
The query-based mask prediction in the $l-1$ layer is 
\begin{align}
    M^{l-1} & = \sigma (F \cdot \text{MLP}(X^{l-1})^T) > 0.5 \nonumber \\
            & = (F \cdot \text{MLP}(X^{l-1})^T > 0 \nonumber
\end{align}
where $F\in R^{T\times H\times W\times D}$ refers to the mask features, and $ \text{MLP}(X^{l-1}) \in R^{N\times D}$ denotes the $N$ predicted mask parameters. The activated function $\sigma$ employs the Sigmoid function.
The $i^{th}$ predicted masks at feature location $(t, x, y)$ is
\begin{align}
    M^{l-1}_n(t, x, y) & =(F(t, x, y) \cdot \text{MLP}(X^{l-1}_i)^T \nonumber \\
                       & = |F(t, x, y)| \cdot |\text{MLP}(X^{l-1}_n)| \nonumber\\
                       &\quad\ cos(F(t, x, y), \text{MLP}(X^{l-1}_n))
\end{align}
Due to $|\cdot| \geq 0$, $M^{l-1}_n(t, x, y) > 0$ equals to $cos(F(t, x, y), \text{MLP}(X^{l-1}_n)) > 0$. Given the predicted masks of the last layer, masked attention knows all possible locations of the instance. 

\begin{table*}
\begin{center}
\begin{tabular}{p{0.15\textwidth}p{0.07\textwidth}<{\centering}|p{0.05\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.09\textwidth}<{\centering}p{0.09\textwidth}<{\centering}|p{0.07\textwidth}p{0.07\textwidth}}
\hline
\multirow{2}{*}{Methods} & \multirow{2}{*}{Sup.} & \multicolumn{5}{c|}{Training Data} & \multicolumn{1}{l}{ytvis21} & \multicolumn{1}{l}{ovis}\\
                         & & ytvis21 & ovis & coco & num. insts & anno. time & val-sub & val-sub   \\
\hline\hline
\multirow{2}{*}{MinVIS} 
& Mask & $\checkmark$  & $\checkmark$ &               & 504k  & 462d & 49.4  & 21.4  \\
& Mask & $\checkmark$  & $\checkmark$ & $\checkmark$  & 831k  & 762d & 51.6{\color{blue} $^{+2.2}$}  & 23.2{\color{blue} $^{+1.8}$}  \\
\hline
\multirow{2}{*}{Mask2Former-video} 
& Mask & $\checkmark$  & $\checkmark$ &               & 504k  & 462d & 50.1  & 22.9  \\
& Mask & $\checkmark$  & $\checkmark$ & $\checkmark$  & 831k  & 762d & 50.3{\color{blue} $^{+0.2}$}  & 26.1{\color{blue} $^{+3.2}$}  \\
\hline 
\multirow{2}{*}{BoxVIS-frame}
& Box  & $\checkmark$  & $\checkmark$ &               & 504k  & 41d & 48.3 & 18.7 \\
& Box  & $\checkmark$  & $\checkmark$ & $\checkmark$  & 831k  & 67d & 48.9{\color{blue} $^{+0.6}$} & 19.2{\color{blue} $^{+0.5}$} \\
\hline
\multirow{2}{*}{BoxVIS-clip}
& Box  & $\checkmark$  & $\checkmark$ &              & 504k  & 41d & 47.5 & 21.8 \\
& Box  & $\checkmark$  & $\checkmark$ & $\checkmark$ & 831k  & 67d & 48.7{\color{blue} $^{+1.3}$}  & 23.3{\color{blue} $^{+1.5}$} \\
\hline
\multirow{2}{*}{+temp. pair}
& Box  & $\checkmark$  & $\checkmark$ &              & 504k  & 41d &  \\
& Box  & $\checkmark$  & $\checkmark$ & $\checkmark$ & 831k  & 67d &  48.8 & 24.2 \\
\hline\hline
\end{tabular}
\end{center}
\caption{Results comparison of SOTA methods with our proposed joint training on BJVIS data set. }
\end{table*}

\begin{table}
\centering
\begin{tabular}{p{0.04\textwidth}<{\centering}p{0.02\textwidth}<{\centering}p{0.04\textwidth}<{\centering}p{0.02\textwidth}<{\centering}|p{0.06\textwidth}<{\centering}p{0.06\textwidth}<{\centering}p{0.04\textwidth}<{\centering}}
\Xhline{0.8pt}
\multicolumn{4}{c|}{Affinity} & \multicolumn{3}{c}{Mask AP}\\
$S_{lab}$ & $k_{lab}$  & $S_{corr}$ & $k_{corr}$ & {\small YTVIS21} &{\small OVIS}  & {\small BVISD}\ \\
\Xhline{0.8pt}
 $\checkmark$ & 1 &              &   &      &      & 33.7 \\
 $\checkmark$ & 3 &              &   &      &      & \\
              &   & $\checkmark$ & 1 &      &      & 32.1 \\ 
              &   & $\checkmark$ & 3 &      &      &      \\ 
 $\checkmark$ & 1 & $\checkmark$ & 1 &      &      & 33.0 \\
 $\checkmark$ & 1 & $\checkmark$ & 3 &      &      & 33.7 \\  
 $\checkmark$ & 3 & $\checkmark$ & 3 &      &      & 32.1 \\ 
 $\checkmark$ & 3 & ms & 3 &      &      & 33.0 \\
% 3 & $\checkmark$ & $\checkmark$ & $\checkmark$ & \\
\Xhline{0.8pt}
\end{tabular}
\caption{Spatial-temporal pairwise affinity loss.}
\end{table}

==> tables/decoder_outputs.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{p{0.08\textwidth}<{\centering}|p{0.16\textwidth}p{0.09\textwidth}p{0.07\textwidth}p{0.07\textwidth}p{0.07\textwidth}p{0.07\textwidth}p{0.07\textwidth}p{0.07\textwidth}}
\hline
  &   &      & \multicolumn{5}{c}{Decoder Layers} \\
Data & Supervision & Metric & 0 & 1 & 2 & 3 & 6 & 9 \\
\hline\hline
\multirow{6}{*}{COCO} & \multirow{2}{*}{Mask}
  & AP$^{box}$  & 1.4 & 39.9 & 42.6 & 44.3 & 45.6 & 45.9 \\
& & AP$^{mask}$ & 1.4 & 37.7 & 40.2 & 41.6{\color {red} $^{+3.9}$} & 42.9$^{+1.3}$ & 43.1$^{+0.2}$ \\
\cline{2-9}
& \multirow{2}{*}{Box (baseline)}
  & AP$^{box}$  & 0.2 & 36.5 & 40.7 & 43.0                        & 45.0          & 45.6 \\
& & AP$^{mask}$ & 0.2 & 30.5 & 34.0 & 35.6{\color {red}$^{+5.1}$} & 37.1$^{+1.5}$ & 37.5$^{+0.4}$ \\
\cline{2-9}
% & \multirow{2}{*}{Box+pseudo(tv)}
  % & Box  AP & 0.63 & 37.3 & & 43.8 & 45.6 & 45.9 \\
% & & Mask AP & 0.55 & 30.8 & & 36.0$^{+5.2}$ & 37.3$^{+1.3}$ & 37.5$^{+0.2}$ \\
\cline{2-9} 
& \multirow{2}{*}{Box + Pseudo Mask}
  & AP$^{box}$  & 0.6 & 38.1 & 42.0 & 44.2                        & 46.2          & 46.5 \\
& & AP$^{mask}$ & 0.5 & 33.0 & 35.9 & 37.7{\color {red}$^{+4.7}$} & 39.0$^{+1.3}$ & 39.2$^{+0.2}$ \\
\hline\hline
\multirow{2}{*}{YT21} 
& Mask + Mask  & AP$^{mask}$ & 1.9 & 25.7 & & 34.8{\color {red}$^{+9.1}$} & 35.6$^{+0.8}$ & 36.8$^{+1.2}$\\
& Mask + Box   & AP$^{mask}$ & 0.6 & 23.9 & & 34.1{\color {red}$^{+10.2}$} & 34.5$^{+0.4}$ & 35.8$^{+1.3}$ \\
\hline
\end{tabular}
\end{center}
\caption{Performance predicted from different decoder layers. Box-supervised baseline employs the projection and pairwise affinity losses proposed in \cite{tian2020boxinst}.} \label{tab:sota_coco}
\end{table*}

==> tables/loss_compare.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{p{0.12\textwidth}<{\centering}p{0.18\textwidth}<{\centering}p{0.22\textwidth}p{0.3\textwidth}}
\hline
Methods & Supervision & Matching loss & Training loss \\
\hline\hline
\multirow{3}{*}{BoxInst} 
& Mask  &  \multirow{3}{*}{$BIoU(A, B) > 0.5$} & $L_{cls}+L_{box}+L_{mask}$\\
& Box   &              & $L_{cls}+L_{box}+L_{proj}+L_{pair}$ \\
& Box+Mask$_{pseu}$ &  & $L_{cls}+L_{box}+L_{proj}+L_{pair}+L_{mask}$ \\
\hline
\multirow{3}{*}{Mask2Former} 
& Mask  & $L_{cls}+L_{mask}$ & $L_{cls}+L_{mask}$ \\
& Box   & $L_{cls}+L_{proj}$ & $L_{cls}+L_{proj}+L_{pair}$ \\
& Box+Mask$_{pseu}$ & $L_{cls}+L_{proj}+L_{mask}$ & $L_{cls}+L_{proj}+L_{pair}+L_{mask}$ \\
\hline
\end{tabular}
\end{center}
\caption{Loss comparison.} \label{tab:sota_coco}
\end{table*}

==> tables/sota_swinl_yt.tex <==
\begin{table}[t]
{\normalsize
\setlength{\tabcolsep}{0.5mm}{
      \linespread{2}
      \begin{tabular}
      {p{0.125\textwidth}p{0.055\textwidth}<{\centering}p{0.05\textwidth}<{\centering}p{0.05\textwidth}<{\centering}p{0.05\textwidth}<{\centering}p{0.05\textwidth}<{\centering}p{0.055\textwidth}<{\centering}}
        \Xhline{0.8pt}
         Method & Super. &\ AP\  &\ AP$_{50}$\ &\ AP$_{75}$\ &\ AR$_{1}$\ &\ AR$_{10}$\ \\
         % \Xhline{1pt}
         % \multirow{4}{*}{\shortstack{YT19}}
         % & SeqFromer\cite{seqformer}             & 59.3 & 82.1 & 66.4 &51.7 &64.4\\
         % & Mask2Former-VIS                       & 60.4 & 84.4 & 67.0 & –   & – \\
         % & MinVIS \cite{huang2022minvis}         & 61.6 & 83.3 & 68.6 &54.8 & 66.6 \\
         % & IDOL \cite{IDOL}                      & 64.3 & 87.5 & 71.0 &55.6 & 69.1 \\
         % & VITA \cite{heo2022vita}               & 63.0 & 86.9 & 67.9 &56.3 & 68.1 \\
         \Xhline{0.8pt}
         % \multicolumn{3}{l}{\textit{\color{blue} YTVIS21}} \\
         % \hline
         {\normalsize SeqFromer}\cite{seqformer}       & Pixel & 51.8 & 74.6 & 58.2 & 42.8 & 58.1 \\
         {\normalsize IDOL} \cite{IDOL}                & Pixel & 56.1 & 80.8 & 63.5 & 45.0  &60.1 \\
         {\normalsize MinVIS} \cite{huang2022minvis}   & Pixel & 55.3 & 76.6 & 62.0 & 45.9 & 60.8 \\
         {\normalsize M2F-VIS} \cite{cheng2021mask2former-video} & pixel  & 40.6 & 60.9 & 41.8 & - & -\\
         {\normalsize VITA} \cite{heo2022vita}         & Pixel & 57.5 & 80.6 & 61.0 & 47.7 & 62.6 \\
         {\normalsize BoxVIS}                          & Box   & \\
         \Xhline{0.8pt}
         % \multicolumn{3}{l}{\textit{ \color{blue} YTVIS22L}} \\
         % \hline
         % IDOL \cite{IDOL}                    & pixel & 40.3 & 64.5 & 41.8 & 33.2 & 45.4 \\
         % MinVIS \cite{huang2022minvis}       & pixel & 33.1 & 54.9 & 33.7 & 29.5 & 36.6 \\
         % M2F-VIS \cite{cheng2021mask2former-video} & pixel &  \\
         % VITA \cite{heo2022vita}             & pixel & 41.1 & 62.9 & 44.0 & 39.3 & 44.3 \\
         % BoxVIS                              & box & \\
         % \Xhline{1pt}
      \end{tabular}
}
}
\vspace{-2mm}
\caption{ Quantitative performance comparison of pixel-supervised and box-supervised VIS methods with Swin Large (SwinL) backbone \cite{vaswani2017attention} on YTVIS21. 
% Symbol "$^\dag$" means that the input video is of 720p.
}\label{tab:sota_swinl_yt}
\end{table}


==> tables/stoa_coco.tex <==
\begin{table}
\begin{center}
\begin{tabular}{p{0.14\textwidth}p{0.025\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.03\textwidth}<{\centering}p{0.025\textwidth}<{\centering}p{0.025\textwidth}<{\centering}p{0.025\textwidth}<{\centering}}
\Xhline{1pt}
Methods & AP & AP$_{50}$ & AP$_{75}$ & AP$_s$ & AP$_m$ & AP$_l$ \\
\Xhline{1pt}
\multicolumn{3}{l}{\textit{ \color{red} Pixel-wise annotations}} \\
CondInst\cite{tian2020conditional}    & 35.9  & 57.0  & 38.2  & 19.0  & 38.6  & 46.7 \\
Mask2Former\cite{cheng2021mask2former}& 43.1  & 65.4  & 46.4  & 22.5  & 46.2  & 64.2 \\
\Xhline{1pt}
\multicolumn{3}{l}{\textit{ \color{red} Box annotations}} \\
BoxInst\cite{tian2020boxinst}         & 32.1  & 55.1  & 32.4  & 15.6  & 34.3  & 43.5 \\
BoxTeacher\cite{cheng2022boxteacher}  & 34.4  & 56.5  & 35.9  & 18.8  & 37.5  & 45.0 \\
% COCO val-dev\\
% Mask2Former-Box  &              & Box   & 37.5  & 60.9  & 38.4  & 18.7  & 39.4  & 57.1 \\
% Mask2Former\cite{cheng2021mask2former}$^\dag$ & Swin-L    & Mask2Former & Box & 3×  & \\
{\small Mask2Former-Box}               & 39.2  & 62.1  & 41.4  & 20.3  & 41.5  & 57.9 \\
\Xhline{1pt}
\end{tabular}
\end{center}
\vspace{-1mm}
\caption{Performance comparison of Image Instance Segmentation on COCO. Comparisons with state-of-the-art methods on COCO test-dev. We introduce the original projection and pairwise affinity losses proposed in BoxInst\cite{tian2020boxinst} and the pseudo masks in BoxTeacher\cite{cheng2022boxteacher} into Mask2Former\cite{cheng2021mask2former} as our baseline. All methods are trained with 36 epochs.} \label{tab:sota_coco}
\end{table}

==> tables/week_report.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{p{0.13\textwidth}<{\centering}|p{0.11\textwidth}<{\centering}p{0.07\textwidth}<{\centering}p{0.07\textwidth}<{\centering}}
\hline
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{{ \color{orange} COCO}} \\
        &  Pretrain Sup.   & AP$^{box}$ & AP$^{mask}$  \\
\hline\hline
CondInst    & Mask    & -    & 35.6  \\
Mask2Former & Mask   & 45.9 & 43.1   \\
\hline
BoxInst    & Box     & -    & 30.7  \\
BoxTeacher & Box     & -    & 34.2  \\
Ours       & Box    & 46.5 & 39.2{\color{orange} $^{+5}$} \\
\hline 
\end{tabular}
\end{center}
\caption{Results on COCO val2017 set. }
\end{table*}
